Robust Angular Synchronization via Directed Graph Neural Networks

The angular synchronization problem aims to accurately estimate (up to a constant additive phase) a set of unknown angles $\theta_1, \dots, \theta_n\in[0, 2\pi)$ from $m$ noisy measurements of their offsets $\theta_i-\theta_j \;\mbox{mod} \; 2\pi.$ Applications include, for example, sensor network localization, phase retrieval, and distributed clock synchronization. An extension of the problem to the heterogeneous setting (dubbed $k$-synchronization) is to estimate $k$ groups of angles simultaneously, given noisy observations (with unknown group assignment) from each group. Existing methods for angular synchronization usually perform poorly in high-noise regimes, which are common in applications. In this paper, we leverage neural networks for the angular synchronization problem, and its heterogeneous extension, by proposing GNNSync, a theoretically-grounded end-to-end trainable framework using directed graph neural networks. In addition, new loss functions are devised to encode synchronization objectives. Experimental results on extensive data sets demonstrate that GNNSync attains competitive, and often superior, performance against a comprehensive set of baselines for the angular synchronization problem and its extension, validating the robustness of GNNSync even at high noise levels.

==> figures_tex/ablation_k1_BAO.tex <==

\begin{figure*}[!hbt]
    \centering
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/BAOp5N360stylegamma.pdf}
    \caption{$\text{BAO}_1(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/BAOp5N360stylemulti_normal1.pdf}
    \caption{$\text{BAO}_2(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/BAOp5N360stylemulti_normal0.pdf}
    \caption{$\text{BAO}_3(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/BAOp5N360styleblock_normal6.pdf}
    \caption{$\text{BAO}_4(p=0.05)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/BAOp10N360stylegamma.pdf}
    \caption{$\text{BAO}_1(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/BAOp10N360stylemulti_normal1.pdf}
    \caption{$\text{BAO}_2(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/BAOp10N360stylemulti_normal0.pdf}
    \caption{$\text{BAO}_3(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/BAOp10N360styleblock_normal6.pdf}
    \caption{$\text{BAO}_4(p=0.1)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/BAOp15N360stylegamma.pdf}
    \caption{$\text{BAO}_1(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/BAOp15N360stylemulti_normal1.pdf}
    \caption{$\text{BAO}_2(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/BAOp15N360stylemulti_normal0.pdf}
    \caption{$\text{BAO}_3(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/BAOp15N360styleblock_normal6.pdf}
    \caption{$\text{BAO}_4(p=0.15)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[ht]{\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth,trim=0cm 0cm 0cm 0cm,clip]{ablation_figures/sync_legend_ablation.png}
  \end{subfigure}
    \caption{MSE performance comparison on GNNSync variants on angular synchronization ($k=1$) for BAO models. $p$ is the network density and $\eta$ is the noise level. Error bars indicate one standard deviation. 
    }
    \label{fig:ablation_k1_BAO}
\end{figure*}

==> figures_tex/ablation_k1_RGGO.tex <==

\begin{figure*}[!hbt]
    \centering
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/RGGOp5N360stylegamma.pdf}
    \caption{$\text{RGGO}_1(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/RGGOp5N360stylemulti_normal1.pdf}
    \caption{$\text{RGGO}_2(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/RGGOp5N360stylemulti_normal0.pdf}
    \caption{$\text{RGGO}_3(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/RGGOp5N360styleblock_normal6.pdf}
    \caption{$\text{RGGO}_4(p=0.05)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/RGGOp10N360stylegamma.pdf}
    \caption{$\text{RGGO}_1(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/RGGOp10N360stylemulti_normal1.pdf}
    \caption{$\text{RGGO}_2(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/RGGOp10N360stylemulti_normal0.pdf}
    \caption{$\text{RGGO}_3(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/RGGOp10N360styleblock_normal6.pdf}
    \caption{$\text{RGGO}_4(p=0.1)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/RGGOp15N360stylegamma.pdf}
    \caption{$\text{RGGO}_1(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/RGGOp15N360stylemulti_normal1.pdf}
    \caption{$\text{RGGO}_2(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/RGGOp15N360stylemulti_normal0.pdf}
    \caption{$\text{RGGO}_3(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/RGGOp15N360styleblock_normal6.pdf}
    \caption{$\text{RGGO}_4(p=0.15)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[ht]{\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth,trim=0cm 0cm 0cm 0cm,clip]{ablation_figures/sync_legend_ablation.png}
  \end{subfigure}
    \caption{MSE performance comparison on GNNSync variants on angular synchronization ($k=1$) for RGGO models. $p$ is the network density and $\eta$ is the noise level. Error bars indicate one standard deviation. 
    }
    \label{fig:ablation_k1_RGGO}
\end{figure*}

==> figures_tex/ablation_k2_BAO.tex <==

\begin{figure*}[!hbt]
    \centering
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k2BAOp5N360stylegamma.pdf}
    \caption{$\text{BAO}_1(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k2BAOp5N360stylemulti_normal1.pdf}
    \caption{$\text{BAO}_2(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k2BAOp5N360stylemulti_normal0.pdf}
    \caption{$\text{BAO}_3(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k2BAOp5N360styleblock_normal6.pdf}
    \caption{$\text{BAO}_4(p=0.05)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k2BAOp10N360stylegamma.pdf}
    \caption{$\text{BAO}_1(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k2BAOp10N360stylemulti_normal1.pdf}
    \caption{$\text{BAO}_2(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k2BAOp10N360stylemulti_normal0.pdf}
    \caption{$\text{BAO}_3(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k2BAOp10N360styleblock_normal6.pdf}
    \caption{$\text{BAO}_4(p=0.1)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k2BAOp15N360stylegamma.pdf}
    \caption{$\text{BAO}_1(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k2BAOp15N360stylemulti_normal1.pdf}
    \caption{$\text{BAO}_2(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k2BAOp15N360stylemulti_normal0.pdf}
    \caption{$\text{BAO}_3(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k2BAOp15N360styleblock_normal6.pdf}
    \caption{$\text{BAO}_4(p=0.15)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[ht]{\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth,trim=0cm 0cm 0cm 0cm,clip]{ablation_figures/ksync_legend_ablation.png}
  \end{subfigure}
    \caption{MSE performance comparison on GNNSync variants on $k-$synchronization with $k=2$ for BAO models. $p$ is the network density and $\eta$ is the noise level. Error bars indicate one standard deviation. 
    }
    \label{fig:ablation_k2_BAO}
\end{figure*}

==> figures_tex/ablation_k2_RGGO.tex <==

\begin{figure*}[!hbt]
    \centering
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k2RGGOp5N360stylegamma.pdf}
    \caption{$\text{RGGO}_1(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k2RGGOp5N360stylemulti_normal1.pdf}
    \caption{$\text{RGGO}_2(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k2RGGOp5N360stylemulti_normal0.pdf}
    \caption{$\text{RGGO}_3(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k2RGGOp5N360styleblock_normal6.pdf}
    \caption{$\text{RGGO}_4(p=0.05)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k2RGGOp10N360stylegamma.pdf}
    \caption{$\text{RGGO}_1(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k2RGGOp10N360stylemulti_normal1.pdf}
    \caption{$\text{RGGO}_2(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k2RGGOp10N360stylemulti_normal0.pdf}
    \caption{$\text{RGGO}_3(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k2RGGOp10N360styleblock_normal6.pdf}
    \caption{$\text{RGGO}_4(p=0.1)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k2RGGOp15N360stylegamma.pdf}
    \caption{$\text{RGGO}_1(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k2RGGOp15N360stylemulti_normal1.pdf}
    \caption{$\text{RGGO}_2(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k2RGGOp15N360stylemulti_normal0.pdf}
    \caption{$\text{RGGO}_3(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k2RGGOp15N360styleblock_normal6.pdf}
    \caption{$\text{RGGO}_4(p=0.15)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[ht]{\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth,trim=0cm 0cm 0cm 0cm,clip]{ablation_figures/ksync_legend_ablation.png}
  \end{subfigure}
    \caption{MSE performance comparison on GNNSync variants on $k-$synchronization with $k=2$ for RGGO models. $p$ is the network density and $\eta$ is the noise level. Error bars indicate one standard deviation. 
    }
    \label{fig:ablation_k2_RGGO}
\end{figure*}

==> figures_tex/ablation_k3_BAO.tex <==

\begin{figure*}[!hbt]
    \centering
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3BAOp5N360stylegamma.pdf}
    \caption{$\text{BAO}_1(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3BAOp5N360stylemulti_normal1.pdf}
    \caption{$\text{BAO}_2(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3BAOp5N360stylemulti_normal0.pdf}
    \caption{$\text{BAO}_3(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3BAOp5N360styleblock_normal6.pdf}
    \caption{$\text{BAO}_4(p=0.05)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3BAOp10N360stylegamma.pdf}
    \caption{$\text{BAO}_1(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3BAOp10N360stylemulti_normal1.pdf}
    \caption{$\text{BAO}_2(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3BAOp10N360stylemulti_normal0.pdf}
    \caption{$\text{BAO}_3(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3BAOp10N360styleblock_normal6.pdf}
    \caption{$\text{BAO}_4(p=0.1)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3BAOp15N360stylegamma.pdf}
    \caption{$\text{BAO}_1(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3BAOp15N360stylemulti_normal1.pdf}
    \caption{$\text{BAO}_2(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3BAOp15N360stylemulti_normal0.pdf}
    \caption{$\text{BAO}_3(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3BAOp15N360styleblock_normal6.pdf}
    \caption{$\text{BAO}_4(p=0.15)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[ht]{\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth,trim=0cm 0cm 0cm 0cm,clip]{ablation_figures/ksync_legend_ablation.png}
  \end{subfigure}
    \caption{MSE performance comparison on GNNSync variants on $k-$synchronization with $k=3$ for BAO models. $p$ is the network density and $\eta$ is the noise level. Error bars indicate one standard deviation. 
    }
    \label{fig:ablation_k3_BAO}
\end{figure*}

==> figures_tex/ablation_k3_ERO.tex <==

\begin{figure*}[!hbt]
    \centering
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3EROp5N360stylegamma.pdf}
    \caption{$\text{ERO}_1(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3EROp5N360stylemulti_normal1.pdf}
    \caption{$\text{ERO}_2(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3EROp5N360stylemulti_normal0.pdf}
    \caption{$\text{ERO}_3(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3EROp5N360styleblock_normal6.pdf}
    \caption{$\text{ERO}_4(p=0.05)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3EROp10N360stylegamma.pdf}
    \caption{$\text{ERO}_1(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3EROp10N360stylemulti_normal1.pdf}
    \caption{$\text{ERO}_2(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3EROp10N360stylemulti_normal0.pdf}
    \caption{$\text{ERO}_3(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3EROp10N360styleblock_normal6.pdf}
    \caption{$\text{ERO}_4(p=0.1)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3EROp15N360stylegamma.pdf}
    \caption{$\text{ERO}_1(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3EROp15N360stylemulti_normal1.pdf}
    \caption{$\text{ERO}_2(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3EROp15N360stylemulti_normal0.pdf}
    \caption{$\text{ERO}_3(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3EROp15N360styleblock_normal6.pdf}
    \caption{$\text{ERO}_4(p=0.15)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[ht]{\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth,trim=0cm 0cm 0cm 0cm,clip]{ablation_figures/ksync_legend_ablation.png}
  \end{subfigure}
    \caption{MSE performance comparison on GNNSync variants on $k-$synchronization with $k=3$ for ERO models. $p$ is the network density and $\eta$ is the noise level. Error bars indicate one standard deviation. 
    }
    \label{fig:ablation_k3_ERO}
\end{figure*}

==> figures_tex/ablation_k3_RGGO.tex <==

\begin{figure*}[!hbt]
    \centering
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3RGGOp5N360stylegamma.pdf}
    \caption{$\text{RGGO}_1(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3RGGOp5N360stylemulti_normal1.pdf}
    \caption{$\text{RGGO}_2(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3RGGOp5N360stylemulti_normal0.pdf}
    \caption{$\text{RGGO}_3(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3RGGOp5N360styleblock_normal6.pdf}
    \caption{$\text{RGGO}_4(p=0.05)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3RGGOp10N360stylegamma.pdf}
    \caption{$\text{RGGO}_1(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3RGGOp10N360stylemulti_normal1.pdf}
    \caption{$\text{RGGO}_2(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3RGGOp10N360stylemulti_normal0.pdf}
    \caption{$\text{RGGO}_3(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3RGGOp10N360styleblock_normal6.pdf}
    \caption{$\text{RGGO}_4(p=0.1)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3RGGOp15N360stylegamma.pdf}
    \caption{$\text{RGGO}_1(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3RGGOp15N360stylemulti_normal1.pdf}
    \caption{$\text{RGGO}_2(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3RGGOp15N360stylemulti_normal0.pdf}
    \caption{$\text{RGGO}_3(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k3RGGOp15N360styleblock_normal6.pdf}
    \caption{$\text{RGGO}_4(p=0.15)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[ht]{\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth,trim=0cm 0cm 0cm 0cm,clip]{ablation_figures/ksync_legend_ablation.png}
  \end{subfigure}
    \caption{MSE performance comparison on GNNSync variants on $k-$synchronization with $k=3$ for RGGO models. $p$ is the network density and $\eta$ is the noise level. Error bars indicate one standard deviation. 
    }
    \label{fig:ablation_k3_RGGO}
\end{figure*}

==> figures_tex/ablation_k4_BAO.tex <==

\begin{figure*}[!hbt]
    \centering
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4BAOp5N360stylegamma.pdf}
    \caption{$\text{BAO}_1(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4BAOp5N360stylemulti_normal1.pdf}
    \caption{$\text{BAO}_2(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4BAOp5N360stylemulti_normal0.pdf}
    \caption{$\text{BAO}_3(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4BAOp5N360styleblock_normal6.pdf}
    \caption{$\text{BAO}_4(p=0.05)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4BAOp10N360stylegamma.pdf}
    \caption{$\text{BAO}_1(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4BAOp10N360stylemulti_normal1.pdf}
    \caption{$\text{BAO}_2(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4BAOp10N360stylemulti_normal0.pdf}
    \caption{$\text{BAO}_3(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4BAOp10N360styleblock_normal6.pdf}
    \caption{$\text{BAO}_4(p=0.1)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4BAOp15N360stylegamma.pdf}
    \caption{$\text{BAO}_1(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4BAOp15N360stylemulti_normal1.pdf}
    \caption{$\text{BAO}_2(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4BAOp15N360stylemulti_normal0.pdf}
    \caption{$\text{BAO}_3(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4BAOp15N360styleblock_normal6.pdf}
    \caption{$\text{BAO}_4(p=0.15)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[ht]{\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth,trim=0cm 0cm 0cm 0cm,clip]{ablation_figures/ksync_legend_ablation.png}
  \end{subfigure}
    \caption{MSE performance comparison on GNNSync variants on $k-$synchronization with $k=4$ for BAO models. $p$ is the network density and $\eta$ is the noise level. Error bars indicate one standard deviation. 
    }
    \label{fig:ablation_k4_BAO}
\end{figure*}

==> figures_tex/ablation_k4_ERO.tex <==

\begin{figure*}[!hbt]
    \centering
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4EROp5N360stylegamma.pdf}
    \caption{$\text{ERO}_1(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4EROp5N360stylemulti_normal1.pdf}
    \caption{$\text{ERO}_2(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4EROp5N360stylemulti_normal0.pdf}
    \caption{$\text{ERO}_3(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4EROp5N360styleblock_normal6.pdf}
    \caption{$\text{ERO}_4(p=0.05)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4EROp10N360stylegamma.pdf}
    \caption{$\text{ERO}_1(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4EROp10N360stylemulti_normal1.pdf}
    \caption{$\text{ERO}_2(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4EROp10N360stylemulti_normal0.pdf}
    \caption{$\text{ERO}_3(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4EROp10N360styleblock_normal6.pdf}
    \caption{$\text{ERO}_4(p=0.1)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4EROp15N360stylegamma.pdf}
    \caption{$\text{ERO}_1(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4EROp15N360stylemulti_normal1.pdf}
    \caption{$\text{ERO}_2(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4EROp15N360stylemulti_normal0.pdf}
    \caption{$\text{ERO}_3(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4EROp15N360styleblock_normal6.pdf}
    \caption{$\text{ERO}_4(p=0.15)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[ht]{\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth,trim=0cm 0cm 0cm 0cm,clip]{ablation_figures/ksync_legend_ablation.png}
  \end{subfigure}
    \caption{MSE performance comparison on GNNSync variants on $k-$synchronization with $k=4$ for ERO models. $p$ is the network density and $\eta$ is the noise level. Error bars indicate one standard deviation. 
    }
    \label{fig:ablation_k4_ERO}
\end{figure*}

==> figures_tex/ablation_k4_RGGO.tex <==

\begin{figure*}[!hbt]
    \centering
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4RGGOp5N360stylegamma.pdf}
    \caption{$\text{RGGO}_1(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4RGGOp5N360stylemulti_normal1.pdf}
    \caption{$\text{RGGO}_2(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4RGGOp5N360stylemulti_normal0.pdf}
    \caption{$\text{RGGO}_3(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4RGGOp5N360styleblock_normal6.pdf}
    \caption{$\text{RGGO}_4(p=0.05)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4RGGOp10N360stylegamma.pdf}
    \caption{$\text{RGGO}_1(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4RGGOp10N360stylemulti_normal1.pdf}
    \caption{$\text{RGGO}_2(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4RGGOp10N360stylemulti_normal0.pdf}
    \caption{$\text{RGGO}_3(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4RGGOp10N360styleblock_normal6.pdf}
    \caption{$\text{RGGO}_4(p=0.1)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4RGGOp15N360stylegamma.pdf}
    \caption{$\text{RGGO}_1(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4RGGOp15N360stylemulti_normal1.pdf}
    \caption{$\text{RGGO}_2(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4RGGOp15N360stylemulti_normal0.pdf}
    \caption{$\text{RGGO}_3(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{ablation_figures/k4RGGOp15N360styleblock_normal6.pdf}
    \caption{$\text{RGGO}_4(p=0.15)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[ht]{\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth,trim=0cm 0cm 0cm 0cm,clip]{ablation_figures/ksync_legend_ablation.png}
  \end{subfigure}
    \caption{MSE performance comparison on GNNSync variants on $k-$synchronization with $k=4$ for RGGO models. $p$ is the network density and $\eta$ is the noise level. Error bars indicate one standard deviation. 
    }
    \label{fig:ablation_k4_RGGO}
\end{figure*}

==> figures_tex/linear_comb_k2_BAO.tex <==
\begin{figure*}[!hbt]
    \centering
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k2BAOp5N360stylegamma.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_1(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k2BAOp5N360stylemulti_normal1.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_2(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k2BAOp5N360stylemulti_normal0.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_3(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k2BAOp5N360styleblock_normal6.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_4(p=0.05)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k2BAOp10N360stylegamma.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_1(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k2BAOp10N360stylemulti_normal1.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_2(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k2BAOp10N360stylemulti_normal0.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_3(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k2BAOp10N360styleblock_normal6.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_4(p=0.1)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k2BAOp15N360stylegamma.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_1(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k2BAOp15N360stylemulti_normal1.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_2(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k2BAOp15N360stylemulti_normal0.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_3(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k2BAOp15N360styleblock_normal6.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_4(p=0.15)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[ht]{\linewidth}
    \centering
    \includegraphics[width=0.9\linewidth,trim=0cm 0cm 0cm 0cm,clip]{linear_comb_figures/linear_comb_legend.png}
  \end{subfigure}
  \vspace{-2mm}
    \caption{MSE comparison on GNNSync variants using as loss $\tau \mathcal{L}_\text{upset}+ \mathcal{L}_\text{cycle}$ with different coefficients $\tau$,  on $k-$synchronization with $k=2$ for BAO models. $p$ is the network density and $\eta$ is the noise level. Error bars indicate one standard deviation. 
    }
    \label{fig:linear_comb_k2_BAO}
\end{figure*}

==> figures_tex/linear_comb_k2_RGGO.tex <==
\begin{figure*}[!hbt]
    \centering
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k2RGGOp5N360stylegamma.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_1(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k2RGGOp5N360stylemulti_normal1.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_2(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k2RGGOp5N360stylemulti_normal0.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_3(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k2RGGOp5N360styleblock_normal6.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_4(p=0.05)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k2RGGOp10N360stylegamma.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_1(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k2RGGOp10N360stylemulti_normal1.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_2(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k2RGGOp10N360stylemulti_normal0.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_3(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k2RGGOp10N360styleblock_normal6.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_4(p=0.1)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k2RGGOp15N360stylegamma.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_1(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k2RGGOp15N360stylemulti_normal1.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_2(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k2RGGOp15N360stylemulti_normal0.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_3(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k2RGGOp15N360styleblock_normal6.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_4(p=0.15)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[ht]{\linewidth}
    \centering
    \includegraphics[width=0.9\linewidth,trim=0cm 0cm 0cm 0cm,clip]{linear_comb_figures/linear_comb_legend.png}
  \end{subfigure}
  \vspace{-2mm}
    \caption{MSE comparison on GNNSync variants using as loss $\tau \mathcal{L}_\text{upset}+ \mathcal{L}_\text{cycle}$ with different coefficients $\tau$,  on $k-$synchronization with $k=2$ for RGGO models. $p$ is the network density and $\eta$ is the noise level. Error bars indicate one standard deviation. 
    }
    \label{fig:linear_comb_k2_RGGO}
\end{figure*}

==> figures_tex/linear_comb_k3_BAO.tex <==
\begin{figure*}[!hbt]
    \centering
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3BAOp5N360stylegamma.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_1(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3BAOp5N360stylemulti_normal1.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_2(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3BAOp5N360stylemulti_normal0.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_3(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3BAOp5N360styleblock_normal6.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_4(p=0.05)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3BAOp10N360stylegamma.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_1(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3BAOp10N360stylemulti_normal1.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_2(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3BAOp10N360stylemulti_normal0.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_3(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3BAOp10N360styleblock_normal6.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_4(p=0.1)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3BAOp15N360stylegamma.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_1(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3BAOp15N360stylemulti_normal1.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_2(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3BAOp15N360stylemulti_normal0.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_3(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3BAOp15N360styleblock_normal6.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_4(p=0.15)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[ht]{\linewidth}
    \centering
    \includegraphics[width=0.9\linewidth,trim=0cm 0cm 0cm 0cm,clip]{linear_comb_figures/linear_comb_legend.png}
  \end{subfigure}
  \vspace{-2mm}
    \caption{MSE comparison on GNNSync variants using as loss $\tau \mathcal{L}_\text{upset}+ \mathcal{L}_\text{cycle}$ with different coefficients $\tau$,  on $k-$synchronization with $k=3$ for BAO models. $p$ is the network density and $\eta$ is the noise level. Error bars indicate one standard deviation. 
    }
    \label{fig:linear_comb_k3_BAO}
\end{figure*}

==> figures_tex/linear_comb_k3_ERO.tex <==
\begin{figure*}[!hbt]
    \centering
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3EROp5N360stylegamma.pdf}
    \vspace{-7mm}
    \caption{$\text{ERO}_1(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3EROp5N360stylemulti_normal1.pdf}
    \vspace{-7mm}
    \caption{$\text{ERO}_2(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3EROp5N360stylemulti_normal0.pdf}
    \vspace{-7mm}
    \caption{$\text{ERO}_3(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3EROp5N360styleblock_normal6.pdf}
    \vspace{-7mm}
    \caption{$\text{ERO}_4(p=0.05)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3EROp10N360stylegamma.pdf}
    \vspace{-7mm}
    \caption{$\text{ERO}_1(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3EROp10N360stylemulti_normal1.pdf}
    \vspace{-7mm}
    \caption{$\text{ERO}_2(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3EROp10N360stylemulti_normal0.pdf}
    \vspace{-7mm}
    \caption{$\text{ERO}_3(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3EROp10N360styleblock_normal6.pdf}
    \vspace{-7mm}
    \caption{$\text{ERO}_4(p=0.1)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3EROp15N360stylegamma.pdf}
    \vspace{-7mm}
    \caption{$\text{ERO}_1(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3EROp15N360stylemulti_normal1.pdf}
    \vspace{-7mm}
    \caption{$\text{ERO}_2(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3EROp15N360stylemulti_normal0.pdf}
    \vspace{-7mm}
    \caption{$\text{ERO}_3(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3EROp15N360styleblock_normal6.pdf}
    \vspace{-7mm}
    \caption{$\text{ERO}_4(p=0.15)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[ht]{\linewidth}
    \centering
    \includegraphics[width=0.9\linewidth,trim=0cm 0cm 0cm 0cm,clip]{linear_comb_figures/linear_comb_legend.png}
  \end{subfigure}
  \vspace{-2mm}
    \caption{MSE comparison on GNNSync variants using as loss $\tau \mathcal{L}_\text{upset}+ \mathcal{L}_\text{cycle}$ with different coefficients $\tau$,  on $k-$synchronization with $k=3$ for ERO models. $p$ is the network density and $\eta$ is the noise level. Error bars indicate one standard deviation. 
    }
    \label{fig:linear_comb_k3_ERO}
\end{figure*}

==> figures_tex/linear_comb_k3_RGGO.tex <==
\begin{figure*}[!hbt]
    \centering
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3RGGOp5N360stylegamma.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_1(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3RGGOp5N360stylemulti_normal1.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_2(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3RGGOp5N360stylemulti_normal0.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_3(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3RGGOp5N360styleblock_normal6.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_4(p=0.05)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3RGGOp10N360stylegamma.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_1(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3RGGOp10N360stylemulti_normal1.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_2(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3RGGOp10N360stylemulti_normal0.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_3(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3RGGOp10N360styleblock_normal6.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_4(p=0.1)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3RGGOp15N360stylegamma.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_1(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3RGGOp15N360stylemulti_normal1.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_2(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3RGGOp15N360stylemulti_normal0.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_3(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k3RGGOp15N360styleblock_normal6.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_4(p=0.15)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[ht]{\linewidth}
    \centering
    \includegraphics[width=0.9\linewidth,trim=0cm 0cm 0cm 0cm,clip]{linear_comb_figures/linear_comb_legend.png}
  \end{subfigure}
  \vspace{-2mm}
    \caption{MSE comparison on GNNSync variants using as loss $\tau \mathcal{L}_\text{upset}+ \mathcal{L}_\text{cycle}$ with different coefficients $\tau$,  on $k-$synchronization with $k=3$ for RGGO models. $p$ is the network density and $\eta$ is the noise level. Error bars indicate one standard deviation. 
    }
    \label{fig:linear_comb_k3_RGGO}
\end{figure*}

==> figures_tex/linear_comb_k4_BAO.tex <==
\begin{figure*}[!hbt]
    \centering
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4BAOp5N360stylegamma.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_1(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4BAOp5N360stylemulti_normal1.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_2(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4BAOp5N360stylemulti_normal0.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_3(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4BAOp5N360styleblock_normal6.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_4(p=0.05)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4BAOp10N360stylegamma.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_1(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4BAOp10N360stylemulti_normal1.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_2(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4BAOp10N360stylemulti_normal0.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_3(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4BAOp10N360styleblock_normal6.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_4(p=0.1)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4BAOp15N360stylegamma.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_1(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4BAOp15N360stylemulti_normal1.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_2(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4BAOp15N360stylemulti_normal0.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_3(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4BAOp15N360styleblock_normal6.pdf}
    \vspace{-7mm}
    \caption{$\text{BAO}_4(p=0.15)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[ht]{\linewidth}
    \centering
    \includegraphics[width=0.9\linewidth,trim=0cm 0cm 0cm 0cm,clip]{linear_comb_figures/linear_comb_legend.png}
  \end{subfigure}
  \vspace{-2mm}
    \caption{MSE comparison on GNNSync variants using as loss $\tau \mathcal{L}_\text{upset}+ \mathcal{L}_\text{cycle}$ with different coefficients $\tau$,  on $k-$synchronization with $k=4$ for BAO models. $p$ is the network density and $\eta$ is the noise level. Error bars indicate one standard deviation. 
    }
    \label{fig:linear_comb_k4_BAO}
\end{figure*}

==> figures_tex/linear_comb_k4_ERO.tex <==
\begin{figure*}[!hbt]
    \centering
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4EROp5N360stylegamma.pdf}
    \vspace{-7mm}
    \caption{$\text{ERO}_1(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4EROp5N360stylemulti_normal1.pdf}
    \vspace{-7mm}
    \caption{$\text{ERO}_2(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4EROp5N360stylemulti_normal0.pdf}
    \vspace{-7mm}
    \caption{$\text{ERO}_3(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4EROp5N360styleblock_normal6.pdf}
    \vspace{-7mm}
    \caption{$\text{ERO}_4(p=0.05)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4EROp10N360stylegamma.pdf}
    \vspace{-7mm}
    \caption{$\text{ERO}_1(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4EROp10N360stylemulti_normal1.pdf}
    \vspace{-7mm}
    \caption{$\text{ERO}_2(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4EROp10N360stylemulti_normal0.pdf}
    \vspace{-7mm}
    \caption{$\text{ERO}_3(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4EROp10N360styleblock_normal6.pdf}
    \vspace{-7mm}
    \caption{$\text{ERO}_4(p=0.1)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4EROp15N360stylegamma.pdf}
    \vspace{-7mm}
    \caption{$\text{ERO}_1(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4EROp15N360stylemulti_normal1.pdf}
    \vspace{-7mm}
    \caption{$\text{ERO}_2(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4EROp15N360stylemulti_normal0.pdf}
    \vspace{-7mm}
    \caption{$\text{ERO}_3(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4EROp15N360styleblock_normal6.pdf}
    \vspace{-7mm}
    \caption{$\text{ERO}_4(p=0.15)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[ht]{\linewidth}
    \centering
    \includegraphics[width=0.9\linewidth,trim=0cm 0cm 0cm 0cm,clip]{linear_comb_figures/linear_comb_legend.png}
  \end{subfigure}
  \vspace{-2mm}
    \caption{MSE comparison on GNNSync variants using as loss $\tau \mathcal{L}_\text{upset}+ \mathcal{L}_\text{cycle}$ with different coefficients $\tau$,  on $k-$synchronization with $k=4$ for ERO models. $p$ is the network density and $\eta$ is the noise level. Error bars indicate one standard deviation. 
    }
    \label{fig:linear_comb_k4_ERO}
\end{figure*}

==> figures_tex/linear_comb_k4_RGGO.tex <==
\begin{figure*}[!hbt]
    \centering
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4RGGOp5N360stylegamma.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_1(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4RGGOp5N360stylemulti_normal1.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_2(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4RGGOp5N360stylemulti_normal0.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_3(p=0.05)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4RGGOp5N360styleblock_normal6.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_4(p=0.05)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4RGGOp10N360stylegamma.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_1(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4RGGOp10N360stylemulti_normal1.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_2(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4RGGOp10N360stylemulti_normal0.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_3(p=0.1)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4RGGOp10N360styleblock_normal6.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_4(p=0.1)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4RGGOp15N360stylegamma.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_1(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4RGGOp15N360stylemulti_normal1.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_2(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4RGGOp15N360stylemulti_normal0.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_3(p=0.15)$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 1.8cm,clip]{linear_comb_figures/k4RGGOp15N360styleblock_normal6.pdf}
    \vspace{-7mm}
    \caption{$\text{RGGO}_4(p=0.15)$}
  \end{subfigure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[ht]{\linewidth}
    \centering
    \includegraphics[width=0.9\linewidth,trim=0cm 0cm 0cm 0cm,clip]{linear_comb_figures/linear_comb_legend.png}
  \end{subfigure}
  \vspace{-2mm}
    \caption{MSE comparison on GNNSync variants using as loss $\tau \mathcal{L}_\text{upset}+ \mathcal{L}_\text{cycle}$ with different coefficients $\tau$,  on $k-$synchronization with $k=4$ for RGGO models. $p$ is the network density and $\eta$ is the noise level. Error bars indicate one standard deviation. 
    }
    \label{fig:linear_comb_k4_RGGO}
\end{figure*}

==> figures_tex/pacm_block_normal6_high.tex <==

\begin{figure*}[!hbt]
    \centering
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GNNSync_k50_thres6_100eta15block_normal6seed2split1.png}
    \caption{GNNSync, $\eta=0.15$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/spectral_k50_thres6_100eta15block_normal6seed2split1.png}
    \caption{Spectral, $\eta=0.15$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/row_norm_spectral_k50_thres6_100eta15block_normal6seed2split1.png}
    \caption{Spectral\_RN, $\eta=0.15$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GPM_k50_thres6_100eta15block_normal6seed2split1.png}
    \caption{GPM, $\eta=0.15$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TranSync_k50_thres6_100eta15block_normal6seed2split1.png}
    \caption{TranSync, $\eta=0.15$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_GCW_k50_thres6_100eta15block_normal6seed2split1.png}
    \caption{CEMP\_GCW, $\eta=0.15$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_MST_k50_thres6_100eta15block_normal6seed2split1.png}
    \caption{CEMP\_MST, $\eta=0.15$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TAS_k50_thres6_100eta15block_normal6seed2split1.png}
    \caption{TAS, $\eta=0.15$}
  \end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GNNSync_k50_thres6_100eta20block_normal6seed2split1.png}
    \caption{GNNSync, $\eta=0.2$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/spectral_k50_thres6_100eta20block_normal6seed2split1.png}
    \caption{Spectral, $\eta=0.2$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/row_norm_spectral_k50_thres6_100eta20block_normal6seed2split1.png}
    \caption{Spectral\_RN, $\eta=0.2$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GPM_k50_thres6_100eta20block_normal6seed2split1.png}
    \caption{GPM, $\eta=0.2$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TranSync_k50_thres6_100eta20block_normal6seed2split1.png}
    \caption{TranSync, $\eta=0.2$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_GCW_k50_thres6_100eta20block_normal6seed2split1.png}
    \caption{CEMP\_GCW, $\eta=0.2$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_MST_k50_thres6_100eta20block_normal6seed2split1.png}
    \caption{CEMP\_MST, $\eta=0.2$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TAS_k50_thres6_100eta20block_normal6seed2split1.png}
    \caption{TAS, $\eta=0.2$}
  \end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GNNSync_k50_thres6_100eta25block_normal6seed2split1.png}
    \caption{GNNSync, $\eta=0.25$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/spectral_k50_thres6_100eta25block_normal6seed2split1.png}
    \caption{Spectral, $\eta=0.25$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/row_norm_spectral_k50_thres6_100eta25block_normal6seed2split1.png}
    \caption{Spectral\_RN, $\eta=0.25$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GPM_k50_thres6_100eta25block_normal6seed2split1.png}
    \caption{GPM, $\eta=0.25$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TranSync_k50_thres6_100eta25block_normal6seed2split1.png}
    \caption{TranSync, $\eta=0.25$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_GCW_k50_thres6_100eta25block_normal6seed2split1.png}
    \caption{CEMP\_GCW, $\eta=0.25$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_MST_k50_thres6_100eta25block_normal6seed2split1.png}
    \caption{CEMP\_MST, $\eta=0.25$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TAS_k50_thres6_100eta25block_normal6seed2split1.png}
    \caption{TAS, $\eta=0.25$}
  \end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \caption{Result visualization for the Sensor Network Localization task on the PACM point cloud using option ``4" as ground-truth angles for high-noise input data. Red dots indicate ground-truth locations and blue dots are estimated city locations.
    }
    \label{fig:pacm_block_normal6_full_high}
\end{figure*}

==> figures_tex/pacm_block_normal6_low.tex <==

\begin{figure*}[!hbt]
    \centering
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GNNSync_k50_thres6_100eta0block_normal6seed2split1.png}
    \caption{GNNSync, $\eta=0$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/spectral_k50_thres6_100eta0block_normal6seed2split1.png}
    \caption{Spectral, $\eta=0$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/row_norm_spectral_k50_thres6_100eta0block_normal6seed2split1.png}
    \caption{Spectral\_RN, $\eta=0$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GPM_k50_thres6_100eta0block_normal6seed2split1.png}
    \caption{GPM, $\eta=0$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TranSync_k50_thres6_100eta0block_normal6seed2split1.png}
    \caption{TranSync, $\eta=0$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_GCW_k50_thres6_100eta0block_normal6seed2split1.png}
    \caption{CEMP\_GCW, $\eta=0$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_MST_k50_thres6_100eta0block_normal6seed2split1.png}
    \caption{CEMP\_MST, $\eta=0$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TAS_k50_thres6_100eta0block_normal6seed2split1.png}
    \caption{TAS, $\eta=0$}
  \end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GNNSync_k50_thres6_100eta5block_normal6seed2split1.png}
    \caption{GNNSync, $\eta=0.05$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/spectral_k50_thres6_100eta5block_normal6seed2split1.png}
    \caption{Spectral, $\eta=0.05$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/row_norm_spectral_k50_thres6_100eta5block_normal6seed2split1.png}
    \caption{Spectral\_RN, $\eta=0.05$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GPM_k50_thres6_100eta5block_normal6seed2split1.png}
    \caption{GPM, $\eta=0.05$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TranSync_k50_thres6_100eta5block_normal6seed2split1.png}
    \caption{TranSync, $\eta=0.05$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_GCW_k50_thres6_100eta5block_normal6seed2split1.png}
    \caption{CEMP\_GCW, $\eta=0.05$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_MST_k50_thres6_100eta5block_normal6seed2split1.png}
    \caption{CEMP\_MST, $\eta=0.05$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TAS_k50_thres6_100eta5block_normal6seed2split1.png}
    \caption{TAS, $\eta=0.05$}
  \end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GNNSync_k50_thres6_100eta10block_normal6seed2split1.png}
    \caption{GNNSync, $\eta=0.1$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/spectral_k50_thres6_100eta10block_normal6seed2split1.png}
    \caption{Spectral, $\eta=0.1$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/row_norm_spectral_k50_thres6_100eta10block_normal6seed2split1.png}
    \caption{Spectral\_RN, $\eta=0.1$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GPM_k50_thres6_100eta10block_normal6seed2split1.png}
    \caption{GPM, $\eta=0.1$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TranSync_k50_thres6_100eta10block_normal6seed2split1.png}
    \caption{TranSync, $\eta=0.1$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_GCW_k50_thres6_100eta10block_normal6seed2split1.png}
    \caption{CEMP\_GCW, $\eta=0.1$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_MST_k50_thres6_100eta10block_normal6seed2split1.png}
    \caption{CEMP\_MST, $\eta=0.1$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TAS_k50_thres6_100eta10block_normal6seed2split1.png}
    \caption{TAS, $\eta=0.1$}
  \end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \caption{Result visualization for the Sensor Network Localization task on the PACM point cloud using option ``4" as ground-truth angles for low-noise input data. Red dots indicate ground-truth locations and blue dots are estimated city locations.
    }
    \label{fig:pacm_block_normal6_full_low}
\end{figure*}

==> figures_tex/pacm_multi_normal0_high.tex <==

\begin{figure*}[!hbt]
    \centering
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GNNSync_k50_thres6_100eta15multi_normal0seed2split1.png}
    \caption{GNNSync, $\eta=0.15$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/spectral_k50_thres6_100eta15multi_normal0seed2split1.png}
    \caption{Spectral, $\eta=0.15$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/row_norm_spectral_k50_thres6_100eta15multi_normal0seed2split1.png}
    \caption{Spectral\_RN, $\eta=0.15$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GPM_k50_thres6_100eta15multi_normal0seed2split1.png}
    \caption{GPM, $\eta=0.15$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TranSync_k50_thres6_100eta15multi_normal0seed2split1.png}
    \caption{TranSync, $\eta=0.15$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_GCW_k50_thres6_100eta15multi_normal0seed2split1.png}
    \caption{CEMP\_GCW, $\eta=0.15$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_MST_k50_thres6_100eta15multi_normal0seed2split1.png}
    \caption{CEMP\_MST, $\eta=0.15$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TAS_k50_thres6_100eta15multi_normal0seed2split1.png}
    \caption{TAS, $\eta=0.15$}
  \end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GNNSync_k50_thres6_100eta20multi_normal0seed2split1.png}
    \caption{GNNSync, $\eta=0.2$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/spectral_k50_thres6_100eta20multi_normal0seed2split1.png}
    \caption{Spectral, $\eta=0.2$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/row_norm_spectral_k50_thres6_100eta20multi_normal0seed2split1.png}
    \caption{Spectral\_RN, $\eta=0.2$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GPM_k50_thres6_100eta20multi_normal0seed2split1.png}
    \caption{GPM, $\eta=0.2$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TranSync_k50_thres6_100eta20multi_normal0seed2split1.png}
    \caption{TranSync, $\eta=0.2$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_GCW_k50_thres6_100eta20multi_normal0seed2split1.png}
    \caption{CEMP\_GCW, $\eta=0.2$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_MST_k50_thres6_100eta20multi_normal0seed2split1.png}
    \caption{CEMP\_MST, $\eta=0.2$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TAS_k50_thres6_100eta20multi_normal0seed2split1.png}
    \caption{TAS, $\eta=0.2$}
  \end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GNNSync_k50_thres6_100eta25multi_normal0seed2split1.png}
    \caption{GNNSync, $\eta=0.25$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/spectral_k50_thres6_100eta25multi_normal0seed2split1.png}
    \caption{Spectral, $\eta=0.25$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/row_norm_spectral_k50_thres6_100eta25multi_normal0seed2split1.png}
    \caption{Spectral\_RN, $\eta=0.25$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GPM_k50_thres6_100eta25multi_normal0seed2split1.png}
    \caption{GPM, $\eta=0.25$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TranSync_k50_thres6_100eta25multi_normal0seed2split1.png}
    \caption{TranSync, $\eta=0.25$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_GCW_k50_thres6_100eta25multi_normal0seed2split1.png}
    \caption{CEMP\_GCW, $\eta=0.25$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_MST_k50_thres6_100eta25multi_normal0seed2split1.png}
    \caption{CEMP\_MST, $\eta=0.25$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TAS_k50_thres6_100eta25multi_normal0seed2split1.png}
    \caption{TAS, $\eta=0.25$}
  \end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \caption{Result visualization for the Sensor Network Localization task on the PACM point cloud using option ``3" as ground-truth angles for high-noise input data. Red dots indicate ground-truth locations and blue dots are estimated city locations.
    }
    \label{fig:pacm_multi_normal0_full_high}
\end{figure*}

==> figures_tex/pacm_multi_normal0_low.tex <==

\begin{figure*}[!hbt]
    \centering
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GNNSync_k50_thres6_100eta0multi_normal0seed2split1.png}
    \caption{GNNSync, $\eta=0$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/spectral_k50_thres6_100eta0multi_normal0seed2split1.png}
    \caption{Spectral, $\eta=0$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/row_norm_spectral_k50_thres6_100eta0multi_normal0seed2split1.png}
    \caption{Spectral\_RN, $\eta=0$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GPM_k50_thres6_100eta0multi_normal0seed2split1.png}
    \caption{GPM, $\eta=0$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TranSync_k50_thres6_100eta0multi_normal0seed2split1.png}
    \caption{TranSync, $\eta=0$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_GCW_k50_thres6_100eta0multi_normal0seed2split1.png}
    \caption{CEMP\_GCW, $\eta=0$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_MST_k50_thres6_100eta0multi_normal0seed2split1.png}
    \caption{CEMP\_MST, $\eta=0$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TAS_k50_thres6_100eta0multi_normal0seed2split1.png}
    \caption{TAS, $\eta=0$}
  \end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GNNSync_k50_thres6_100eta5multi_normal0seed2split1.png}
    \caption{GNNSync, $\eta=0.05$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/spectral_k50_thres6_100eta5multi_normal0seed2split1.png}
    \caption{Spectral, $\eta=0.05$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/row_norm_spectral_k50_thres6_100eta5multi_normal0seed2split1.png}
    \caption{Spectral\_RN, $\eta=0.05$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GPM_k50_thres6_100eta5multi_normal0seed2split1.png}
    \caption{GPM, $\eta=0.05$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TranSync_k50_thres6_100eta5multi_normal0seed2split1.png}
    \caption{TranSync, $\eta=0.05$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_GCW_k50_thres6_100eta5multi_normal0seed2split1.png}
    \caption{CEMP\_GCW, $\eta=0.05$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_MST_k50_thres6_100eta5multi_normal0seed2split1.png}
    \caption{CEMP\_MST, $\eta=0.05$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TAS_k50_thres6_100eta5multi_normal0seed2split1.png}
    \caption{TAS, $\eta=0.05$}
  \end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GNNSync_k50_thres6_100eta10multi_normal0seed2split1.png}
    \caption{GNNSync, $\eta=0.1$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/spectral_k50_thres6_100eta10multi_normal0seed2split1.png}
    \caption{Spectral, $\eta=0.1$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/row_norm_spectral_k50_thres6_100eta10multi_normal0seed2split1.png}
    \caption{Spectral\_RN, $\eta=0.1$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GPM_k50_thres6_100eta10multi_normal0seed2split1.png}
    \caption{GPM, $\eta=0.1$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TranSync_k50_thres6_100eta10multi_normal0seed2split1.png}
    \caption{TranSync, $\eta=0.1$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_GCW_k50_thres6_100eta10multi_normal0seed2split1.png}
    \caption{CEMP\_GCW, $\eta=0.1$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_MST_k50_thres6_100eta10multi_normal0seed2split1.png}
    \caption{CEMP\_MST, $\eta=0.1$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TAS_k50_thres6_100eta10multi_normal0seed2split1.png}
    \caption{TAS, $\eta=0.1$}
  \end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \caption{Result visualization for the Sensor Network Localization task on the PACM point cloud using option ``3" as ground-truth angles for low-noise input data. Red dots indicate ground-truth locations and blue dots are estimated city locations.
    }
    \label{fig:pacm_multi_normal0_full_low}
\end{figure*}

==> figures_tex/pacm_multi_normal1_high.tex <==

\begin{figure*}[!hbt]
    \centering
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GNNSync_k50_thres6_100eta15multi_normal1seed2split1.png}
    \caption{GNNSync, $\eta=0.15$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/spectral_k50_thres6_100eta15multi_normal1seed2split1.png}
    \caption{Spectral, $\eta=0.15$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/row_norm_spectral_k50_thres6_100eta15multi_normal1seed2split1.png}
    \caption{Spectral\_RN, $\eta=0.15$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GPM_k50_thres6_100eta15multi_normal1seed2split1.png}
    \caption{GPM, $\eta=0.15$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TranSync_k50_thres6_100eta15multi_normal1seed2split1.png}
    \caption{TranSync, $\eta=0.15$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_GCW_k50_thres6_100eta15multi_normal1seed2split1.png}
    \caption{CEMP\_GCW, $\eta=0.15$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_MST_k50_thres6_100eta15multi_normal1seed2split1.png}
    \caption{CEMP\_MST, $\eta=0.15$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TAS_k50_thres6_100eta15multi_normal1seed2split1.png}
    \caption{TAS, $\eta=0.15$}
  \end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GNNSync_k50_thres6_100eta20multi_normal1seed2split1.png}
    \caption{GNNSync, $\eta=0.2$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/spectral_k50_thres6_100eta20multi_normal1seed2split1.png}
    \caption{Spectral, $\eta=0.2$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/row_norm_spectral_k50_thres6_100eta20multi_normal1seed2split1.png}
    \caption{Spectral\_RN, $\eta=0.2$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GPM_k50_thres6_100eta20multi_normal1seed2split1.png}
    \caption{GPM, $\eta=0.2$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TranSync_k50_thres6_100eta20multi_normal1seed2split1.png}
    \caption{TranSync, $\eta=0.2$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_GCW_k50_thres6_100eta20multi_normal1seed2split1.png}
    \caption{CEMP\_GCW, $\eta=0.2$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_MST_k50_thres6_100eta20multi_normal1seed2split1.png}
    \caption{CEMP\_MST, $\eta=0.2$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TAS_k50_thres6_100eta20multi_normal1seed2split1.png}
    \caption{TAS, $\eta=0.2$}
  \end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GNNSync_k50_thres6_100eta25multi_normal1seed2split1.png}
    \caption{GNNSync, $\eta=0.25$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/spectral_k50_thres6_100eta25multi_normal1seed2split1.png}
    \caption{Spectral, $\eta=0.25$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/row_norm_spectral_k50_thres6_100eta25multi_normal1seed2split1.png}
    \caption{Spectral\_RN, $\eta=0.25$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GPM_k50_thres6_100eta25multi_normal1seed2split1.png}
    \caption{GPM, $\eta=0.25$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TranSync_k50_thres6_100eta25multi_normal1seed2split1.png}
    \caption{TranSync, $\eta=0.25$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_GCW_k50_thres6_100eta25multi_normal1seed2split1.png}
    \caption{CEMP\_GCW, $\eta=0.25$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_MST_k50_thres6_100eta25multi_normal1seed2split1.png}
    \caption{CEMP\_MST, $\eta=0.25$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TAS_k50_thres6_100eta25multi_normal1seed2split1.png}
    \caption{TAS, $\eta=0.25$}
  \end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \caption{Result visualization for the Sensor Network Localization task on the PACM point cloud using option ``2" as ground-truth angles for high-noise input data. Red dots indicate ground-truth locations and blue dots are estimated city locations.
    }
    \label{fig:pacm_multi_normal1_full_high}
\end{figure*}

==> figures_tex/pacm_multi_normal1_low.tex <==

\begin{figure*}[!hbt]
    \centering
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GNNSync_k50_thres6_100eta0multi_normal1seed2split1.png}
    \caption{GNNSync, $\eta=0$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/spectral_k50_thres6_100eta0multi_normal1seed2split1.png}
    \caption{Spectral, $\eta=0$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/row_norm_spectral_k50_thres6_100eta0multi_normal1seed2split1.png}
    \caption{Spectral\_RN, $\eta=0$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GPM_k50_thres6_100eta0multi_normal1seed2split1.png}
    \caption{GPM, $\eta=0$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TranSync_k50_thres6_100eta0multi_normal1seed2split1.png}
    \caption{TranSync, $\eta=0$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_GCW_k50_thres6_100eta0multi_normal1seed2split1.png}
    \caption{CEMP\_GCW, $\eta=0$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_MST_k50_thres6_100eta0multi_normal1seed2split1.png}
    \caption{CEMP\_MST, $\eta=0$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TAS_k50_thres6_100eta0multi_normal1seed2split1.png}
    \caption{TAS, $\eta=0$}
  \end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GNNSync_k50_thres6_100eta5multi_normal1seed2split1.png}
    \caption{GNNSync, $\eta=0.05$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/spectral_k50_thres6_100eta5multi_normal1seed2split1.png}
    \caption{Spectral, $\eta=0.05$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/row_norm_spectral_k50_thres6_100eta5multi_normal1seed2split1.png}
    \caption{Spectral\_RN, $\eta=0.05$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GPM_k50_thres6_100eta5multi_normal1seed2split1.png}
    \caption{GPM, $\eta=0.05$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TranSync_k50_thres6_100eta5multi_normal1seed2split1.png}
    \caption{TranSync, $\eta=0.05$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_GCW_k50_thres6_100eta5multi_normal1seed2split1.png}
    \caption{CEMP\_GCW, $\eta=0.05$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_MST_k50_thres6_100eta5multi_normal1seed2split1.png}
    \caption{CEMP\_MST, $\eta=0.05$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TAS_k50_thres6_100eta5multi_normal1seed2split1.png}
    \caption{TAS, $\eta=0.05$}
  \end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GNNSync_k50_thres6_100eta10multi_normal1seed2split1.png}
    \caption{GNNSync, $\eta=0.1$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/spectral_k50_thres6_100eta10multi_normal1seed2split1.png}
    \caption{Spectral, $\eta=0.1$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/row_norm_spectral_k50_thres6_100eta10multi_normal1seed2split1.png}
    \caption{Spectral\_RN, $\eta=0.1$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/GPM_k50_thres6_100eta10multi_normal1seed2split1.png}
    \caption{GPM, $\eta=0.1$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TranSync_k50_thres6_100eta10multi_normal1seed2split1.png}
    \caption{TranSync, $\eta=0.1$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_GCW_k50_thres6_100eta10multi_normal1seed2split1.png}
    \caption{CEMP\_GCW, $\eta=0.1$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/CEMP_MST_k50_thres6_100eta10multi_normal1seed2split1.png}
    \caption{CEMP\_MST, $\eta=0.1$}
  \end{subfigure}
  \begin{subfigure}[ht]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm,clip]{pacm_figures/TAS_k50_thres6_100eta10multi_normal1seed2split1.png}
    \caption{TAS, $\eta=0.1$}
  \end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \caption{Result visualization for the Sensor Network Localization task on the PACM point cloud using option ``2" as ground-truth angles for low-noise input data. Red dots indicate ground-truth locations and blue dots are estimated city locations.
    }
    \label{fig:pacm_multi_normal1_full_low}
\end{figure*}
